Elaborating Intersection and Union Types

Designing and implementing typed programming languages is hard. Every new type system feature requires extending the metatheory and implementation, which are often complicated and fragile. To ease this process, we would like to provide general mechanisms that subsume many different features. In modern type systems, parametric polymorphism is fundamental, but intersection polymorphism has gained little traction in programming languages. Most practical intersection type systems have supported only refinement intersections, which increase the expressiveness of types (more precise properties can be checked) without altering the expressiveness of terms; refinement intersections can simply be erased during compilation. In contrast, unrestricted intersections increase the expressiveness of terms, and can be used to encode diverse language features, promising an economy of both theory and implementation. We describe a foundation for compiling unrestricted intersection and union types: an elaboration type system that generates ordinary lambda-calculus terms. The key feature is a Forsythe-like merge construct. With this construct, not all reductions of the source program preserve types; however, we prove that ordinary call-by-value evaluation of the elaborated program corresponds to a type-preserving evaluation of the source program. We also describe a prototype implementation and applications of unrestricted intersections and unions: records, operator overloading, and simulating dynamic typing.

==> catmac.tex <==
%

%
%
%
%
%

%
%
%
%

%
%


%

\newcount\yyitercn %
\newcount\yycnA %

\newbox\yybxA %
%
\newbox\yybxB %
\newbox\yybxC %
\newbox\yybxD %
\newbox\yybxE %
\newbox\yybxF %
\newbox\yybxG %

\newdimen\yydmA %
%
\newdimen\yydmB %
\newdimen\yydmC %
\newdimen\yydmD %
\newdimen\yydmE %
\newdimen\yydmF %
\newdimen\yydmG %
\newdimen\yydmH %
\newdimen\yydmI %



%

%
%
%
%
%
%
%

\def\defaxis#1#2{\setbox\yybxA=\hbox{{$#2\vcenter{}$}}
\edef#1{\the\ht\yybxA}}

\defaxis\displayaxis\displaystyle
\defaxis\textaxis\textstyle
\defaxis\scriptaxis\scriptstyle
\defaxis\scriptscriptaxis\scriptscriptstyle

%
%

\def\eqper{\: .}
\def\eqcom{\: ,}

%
%
%
%
%

\def\reflect#1{{#1}^\dagger}
\def\inverse#1{{#1}^{-1}}
\def\dual#1{{#1}^{\rm op}}
\def\identgen#1#2{I^{#1}_{#2}}
\def\ident#1{I_{#1}}

%
%
%
%

%
%

%
%
%
%
%

%

%

%
%
%
%

%
%
%
%
%

\def\domainop{\mathop{\rm dom}\nolimits}
\def\rangeop{\mathop{\rm ran}\nolimits}
\def\sizeop{\mathord{\#}}
\def\objectsop{\mathop{\rm Ob}\nolimits}
\def\morphsop{\mathop{\rm Mor}\nolimits}
\def\apop{\mathop{\sf ap}\nolimits}
\def\abop{\mathop{\sf ab}\nolimits}


%

%
%
%

%
%

\def\restrictop{\mathord{\rceil}}
\def\corestrictop{\mathord{\lceil}}

\def\sccompop{\mathbin{;}}

%
%
%

\def\godmult{\mathbin{\mathchoice
{\kern0.25pt\vrule height7pt depth3.5pt
\vrule height7pt depth-6.6pt width4pt
\kern-4pt\vrule height-3.1pt depth3.5pt width4pt
\kern-3.3pt\textstyle ;\kern-0.03333pt
\vrule height7pt depth3.5pt\kern1pt}
{\kern0.25pt\vrule height7pt depth3.5pt
\vrule height7pt depth-6.6pt width4pt
\kern-4pt\vrule height-3.1pt depth3.5pt width4pt
\kern-3.3pt\textstyle ;\kern-0.03333pt
\vrule height7pt depth3.5pt\kern1pt}
{\kern0.5pt\vrule height5pt depth2.5pt
\vrule height5pt depth-4.6pt width3pt
\kern-3pt\vrule height-2.1pt depth2.5pt width3pt
\kern-2.4pt\scriptstyle ;\kern0.03889pt
\vrule height5pt depth2.5pt\kern1pt}
{\kern0.5pt\vrule height4.25pt depth2pt
\vrule height4.25pt depth-3.85pt width2.75pt
\kern-2.75pt\vrule height-1.6pt depth2pt width2.75pt
\kern-2.275pt\scriptscriptstyle ;\kern-0.00277pt
\vrule height4.25pt depth2pt\kern1pt}}}


%

%
%
%

\def\eqdef{\buildrel \rm def \over =}

\def\noteq{\mathrel{\not=}}

\def\finsubset{\buildrel \rm fin \over \subseteq}

%
%
%
%

%
%

\let\oldin=\in
\let\yyoldnotinraw=\notin %
\def\oldnotin{\mathrel{{\def\in{\oldin}\yyoldnotinraw}}}

\def\in{\mathrel{\mathchoice
{\makelevel{\scriptstyle\oldin}}
{\makelevel{\scriptstyle\oldin}}
{\makelevel{\scriptscriptstyle\oldin}}
{\scriptscriptstyle\oldin}}}

\def\notin{\mathrel{\mathchoice
{\makelevel{\scriptstyle\oldnotin}}
{\makelevel{\scriptstyle\oldnotin}}
{\makelevel{\scriptscriptstyle\oldnotin}}
{\scriptscriptstyle\oldnotin}}}

\def\makelevel#1{\setbox\yybxA=\hbox{$\mathsurround=0pt{#1}$}
\yydmA=\dp\yybxA \raise\yydmA\hbox{$\mathsurround=0pt{#1}$}}

%

\def\uniquein{\mathrel{{\in}!}}

%
%
%
%

%
%
%
%
%
%
%

\def\arrow{\rightarrow}
\def\arrowsub#1{\yyarrowa{_{#1}}}
\def\arrowsuper#1{\yyarrowa{^{#1}}}
\def\arrowsubsuper#1#2{\yyarrowa{_{#1}^{#2}}}

\def\Arrow{\Rightarrow}
\def\Arrowsub#1{\yyArrowa{_{#1}}}
\def\Arrowsuper#1{\yyArrowa{^{#1}}}
\def\Arrowsubsuper#1#2{\yyArrowa{_{#1}^{#2}}}

\def\yyarrowa#1{\mathrel{\mathchoice %
{\yyarrowb\yyrightarrowfill\displaystyle\displayaxis{#1}{0ex}{0ex}
{6mu}{8mu}\rightarrow}
{\yyarrowb\yyrightarrowfill\textstyle\textaxis{#1}{0ex}{0ex}
{6mu}{8mu}\rightarrow}
{\yyarrowb\yyrightarrowfill\scriptstyle\scriptaxis{#1}{0ex}{0ex}
{6mu}{8mu}\rightarrow}
{\yyarrowb\yyrightarrowfill\scriptscriptstyle
\scriptscriptaxis{#1}{0ex}{0ex}{6mu}{8mu}\rightarrow}}}

\def\yyArrowa#1{\mathrel{\mathchoice %
{\yyarrowb\yyRightarrowfill\displaystyle\displayaxis{#1}{0.2ex}{0.2ex}
{6mu}{12mu}\Rightarrow}
{\yyarrowb\yyRightarrowfill\textstyle\textaxis{#1}{0.2ex}{0.2ex}
{6mu}{12mu}\Rightarrow}
{\yyarrowb\yyRightarrowfill\scriptstyle\scriptaxis{#1}{0.1ex}{0ex}
{6mu}{12mu}\Rightarrow}
{\yyarrowb\yyRightarrowfill\scriptscriptstyle
\scriptscriptaxis{#1}{0.1ex}{0ex}{6mu}{12mu}\Rightarrow}}}

\def\yyarrowb#1#2#3#4#5#6#7#8#9{{ %
\setbox\yybxA=\hbox{$\mathsurround=0pt #2
\mkern #7\mathop{}\limits #4\mkern #8$}
\yydmA=\wd\yybxA\relax
\setbox\yybxA=\hbox{$\mathsurround=0pt #2 #9$}
\ifdim\yydmA<\wd\yybxA\relax\yydmA=\wd\yybxA\relax\else\fi
\setbox\yybxA=\hbox to \yydmA{#1 #2}
\yydmA=#3\relax\advance\yydmA by #5\relax\ht\yybxA=\yydmA\relax
\yydmA=-#3\relax\advance\yydmA by #6\relax\dp\yybxA=\yydmA\relax
#2\mathop{\box\yybxA}\limits #4}}

\def\yyrightarrowfill#1{$\mathsurround=0pt #1\mathord- \mkern-9mu %
\cleaders\hbox{$#1\mkern-3mu \mathord- \mkern-3mu$}\hfill
\mkern-9mu \mathord\rightarrow$}

\def\yyRightarrowfill#1{$\mathsurround=0pt #1\mathord= \mkern-9mu %
\cleaders\hbox{$#1\mkern-3mu \mathord= \mkern-3mu$}\hfill
\mkern-9mu \mathord\Rightarrow$}


%

%
%

%
%
%
%

%
%
%
%
%
%
%
%
%
%

\def\defbig#1#2#3#4{\setbox\yybxA=\hbox{$#1#2($}
\yydmA=\ht\yybxA\relax\yydmB=\dp\yybxA\relax\yycnA=50\relax
\yydefbiga{#1}{#3}{#4}}

\def\yydefbiga#1#2#3{\advance\yydmA by 0.2pt\relax %
\advance\yycnA by -1\relax
\setbox\yybxA=\hbox{$#1\left(\vbox to \yydmA{}\right.
\nulldelimiterspace=0pt\mathsurround=0pt$}
\yydmC=\dp\yybxA\relax\advance\yydmC by -\yydmB\relax
\advance\yydmC by -#3\relax
\ifdim\yydmC<0pt\relax\ifnum\yycnA>0\relax
\yydefbiga{#1}{#2}{#3}
\else\yydefbigb{#2}{#1}\fi
\else\yydefbigb{#2}{#1}\fi}

\def\yydefbigb#1#2{\edef\yybigsize{{\the\yydmA}} %
\expandafter\yydefbigc\yybigsize{#1}{#2}}

\def\yydefbigc#1#2#3{\def#2##1{{\hbox{$#3\left##1\vbox to #1{}\right. %
\nulldelimiterspace=0pt\mathsurround=0pt$}}}}

%
%
%
%
%
%
%

\defbig\textstyle\relax\big{0.95pt}
\defbig\textstyle\big\Big{0.95pt}
\defbig\textstyle\Big\bigg{0.95pt}
\defbig\textstyle\bigg\Bigg{0.95pt}

%
%
%

\defbig\scriptstyle\relax\scriptbig{0.95pt}
\defbig\scriptscriptstyle\relax\scriptscriptbig{0.95pt}
\def\scriptbigl{\mathopen\scriptbig}
\def\scriptbigm{\mathrel\scriptbig}
\def\scriptbigr{\mathclose\scriptbig}
\def\scriptscriptbigl{\mathopen\scriptscriptbig}
\def\scriptscriptbigm{\mathrel\scriptscriptbig}
\def\scriptscriptbigr{\mathclose\scriptscriptbig}

%
%
%
%

%
%
%
%

\def\normsize#1{\begingroup\let\currbig=\relax #1\endgroup}
\def\bigsize#1{\begingroup\let\currbig=\big #1\endgroup}
\def\Bigsize#1{\mathinner{{\let\currbig=\Big #1}}}
\def\biggsize#1{\mathinner{{\let\currbig=\bigg #1}}}
\def\Biggsize#1{\mathinner{{\let\currbig=\Bigg #1}}}
\def\scriptbigsize#1{\begingroup\let\currbig=\scriptbig #1\endgroup}
\def\scriptscriptbigsize#1{\begingroup\let\currbig=\scriptscriptbig
#1\endgroup}

%
%
%

\let\currbig=\relax

%
%
%
%

\def\varlpar{\mathopen\currbig(}
\def\varrpar{\mathclose\currbig)}
\def\varlbrack{\mathopen\currbig\lbrack}
\def\varrbrack{\mathclose\currbig\rbrack}
\def\varlbrace{\mathopen\currbig\lbrace}
\def\varrbrace{\mathclose\currbig\rbrace}
\def\varlangle{\mathopen\currbig\langle}
\def\varrangle{\mathclose\currbig\rangle}
\def\varlvert{\mathopen\currbig\vert}
\def\varrvert{\mathclose\currbig\vert}
\def\varmid{\mathrel\currbig\vert}

%
%

%
%

\def\varlsembr{\mathopen{{\currbig\lbrack
\kernpart{\currbig\lbrack}{-59}\currbig\lbrack}}}

\def\varrsembr{\mathclose{{\currbig\rbrack
\kernpart{\currbig\rbrack}{-59}\currbig\rbrack}}}

%

\def\kernpart#1#2{\mathchoice
{\yykernparta{\displaystyle#1}{#2}}
{\yykernparta{\textstyle#1}{#2}}
{\yykernparta{\scriptstyle#1}{#2}}
{\yykernparta{\scriptscriptstyle#1}{#2}}}

\def\yykernparta#1#2{ %
\setbox\yybxA=\hbox{$\mathsurround=0pt\relax #1$}
\yydmA=\wd\yybxA\multiply\yydmA by #2\relax
\divide\yydmA by 100\relax \kern\yydmA}

%

%
%

\def\varbdlangle{\mathopen{{\embolden{\currbig\langle}{.025em}}}}
\def\varbdrangle{\mathclose{{\embolden{\currbig\rangle}{.025em}}}}

%
%

\def\embolden#1#2{\mathchoice
{\yyemboldena{\displaystyle#1}{#2}}
{\yyemboldena{\textstyle#1}{#2}}
{\yyemboldena{\scriptstyle#1}{#2}}
{\yyemboldena{\scriptscriptstyle#1}{#2}}}

\def\yyemboldena#1#2{ %
\setbox\yybxA=\hbox{$\mathsurround=0pt\relax #1$}
\copy\yybxA\kern-\wd\yybxA\kern #2\relax
\raise #2\copy\yybxA\kern-\wd\yybxA\relax
\raise -#2\copy\yybxA\kern-\wd\yybxA\kern #2\relax
\box\yybxA}

%
%
%
%
%
%
%

\def\paren#1{\varlpar\normsize{#1}\varrpar}
\def\carrier#1{\varlvert\normsize{#1}\varrvert}
\def\setdef#1#2{\varlbrace\nonscript\,\normsize{#1}\varmid
\normsize{#2}\nonscript\,\varrbrace}
\def\sembr#1{\varlsembr\normsize{#1}\varrsembr}


%

%
%
%
%

%
%
%
%
%

%
%
%
%
%
%

\def\simplist#1#2#3#4#5{
%
%
%
%
%
\yyitercn=#1\relax
\def\yyrightdel{#3}
\def\yysepsym{#4}
\ifnum\yyitercn=0\relax
#5 \let\next=\relax
\else #2 \let\next=\yysimplista
\fi\next}

\def\yysimplista#1{\begingroup\normsize{#1}\endgroup %
\advance\yyitercn by -1\relax
\ifnum\yyitercn=0\relax
\yyrightdel \let\next=\relax
\else \yysepsym \let\next=\yysimplista
\fi\next}

\def\emptyset{\varlbrace\varrbrace}

\def\setlist#1{\simplist{#1}\varlbrace\varrbrace{,}\emptyset}

\def\emptysqlist{\varlbrack\,\varrbrack}

\def\sqlist#1{\simplist{#1}\varlbrack\varrbrack{,}\emptysqlist}

\def\emptyanglelist{\varlangle\varrangle}

\def\anglelist#1{\simplist{#1}\varlangle\varrangle{,}\emptyanglelist}

\def\emptybdanglelist{\varbdlangle\varbdrangle}

\def\bdanglelist#1{\simplist{#1}\varbdlangle\varbdrangle{,}\emptybdanglelist}

%
%
%
%
%
%
%

%
%
%

%
%
%
%
%
%

%
%

\def\pairlist#1#2#3#4#5#6{
%
%
%
%
%
%
\yyitercn=#1\relax
\def\yyrightdel{#3}
\def\yysepsym{#4}
\def\yypairsym{#5}
\ifnum\yyitercn=0\relax
#6 \let\next=\relax
\else #2 \let\next=\yypairlista
\fi\next}

\def\yypairlista#1#2{ %
\begingroup\normsize{#1}\endgroup\yypairsym
\begingroup\normsize{#2}\endgroup
\advance\yyitercn by -1\relax
\ifnum\yyitercn=0\relax
\yyrightdel \let\next=\relax
\else \yysepsym \let\next=\yypairlista
\fi\next}

\def\pairlistdots#1#2#3#4#5#6#7#8{
%
%
%
%
%
%
%
%
#1\begingroup\normsize{#5}\endgroup #4
\begingroup\normsize{#6}\endgroup #3
\ldots #3\begingroup\normsize{#7}\endgroup #4
\begingroup\normsize{#8}\endgroup #2}

\def\sqpairlist#1{\pairlist{#1}
{\varlbrack\nonscript\,}{\nonscript\,\varrbrack}\varmid\colon\emptysqlist}

\def\sqpairlistdots{\pairlistdots
{\varlbrack\nonscript\,}{\nonscript\,\varrbrack}\varmid\colon}

\def\anglepairlist#1{\pairlist{#1}
{\varlangle\nonscript\,}{\nonscript\,\varrangle}\varmid\colon\emptyanglelist}

\def\anglepairlistdots{\pairlistdots
{\varlangle\nonscript\,}{\nonscript\,\varrangle}\varmid\colon}

\def\bdanglepairlist#1{\pairlist{#1}
{\varbdlangle\nonscript\,}{\nonscript\,\varbdrangle}\varmid\colon
\emptybdanglelist}

\def\bdanglepairlistdots{\pairlistdots
{\varbdlangle\nonscript\,}{\nonscript\,\varbdrangle}\varmid\colon}

%
%
%
%
%

%
%
%

%
%
%
%
%
%

%
%

\def\pairext#1#2#3#4#5#6{
%
%
%
%
%
%
\pairlist{#1}{#2\begingroup\normsize{#6}\endgroup #4}
{#3}{#4}{#5}{#2\begingroup\normsize{#6}\endgroup #3}}

\def\pairextdots#1#2#3#4#5#6#7#8#9{
%
%
%
%
%
%
%
%
%
\pairlistdots{#1\begingroup\normsize{#5}\endgroup #3}
{#2}{#3}{#4}{#6}{#7}{#8}{#9}}

\def\sqpairext#1{\pairext{#1}
{\varlbrack\nonscript\,}{\nonscript\,\varrbrack}\varmid\colon}

\def\sqpairextdots{\pairextdots
{\varlbrack\nonscript\,}{\nonscript\,\varrbrack}\varmid\colon}

\def\anglepairext#1{\pairext{#1}
{\varlangle\nonscript\,}{\nonscript\,\varrangle}\varmid\colon}

\def\anglepairextdots{\pairextdots
{\varlangle\nonscript\,}{\nonscript\,\varrangle}\varmid\colon}

\def\bdanglepairext#1{\pairext{#1}
{\varbdlangle\nonscript\,}{\nonscript\,\varbdrangle}\varmid\colon}

\def\bdanglepairextdots{\pairextdots
{\varbdlangle\nonscript\,}{\nonscript\,\varbdrangle}\varmid\colon}

%
%
%
%
%

%
%

\def\infix#1#2{
%
%
\yyitercn=#1\relax
\def\yysepsym{#2}
\ifnum\yyitercn=0\relax
\errmessage{CALL OF \string\infix0}
\let\next=\relax
\else\let\next=\yyinfixa
\fi\next}

\def\yyinfixa#1{\begingroup #1\endgroup %
\advance\yyitercn by -1\relax
\ifnum\yyitercn=0\relax
\let\next=\relax
\else \yysepsym \let\next=\yyinfixa
\fi\next}

\def\compo#1{\infix{#1}{\sccompop}}
\def\compogen#1#2{\infix{#1}{\sccompop_{\normsize{#2}}}}
\def\fcompo#1{\infix{#1}{\cdot}}
\def\fcompogen#1#2{\infix{#1}{\cdot_{\normsize{#2}}}}
\def\godcompo#1{\infix{#1}{\godmult}}


%

%
%
%

\def\lambin#1#2{\lambda{#1}\in{#2}.\;}

%
%
%
%

\def\emptylambin{\lambda\varlangle\varrangle.\;}

\def\multlambin#1{\pairlist{#1}{\lambda\varlangle\nonscript\,}
{\nonscript\,\varrangle.\;}{,\nonscript\:}\in\emptylambin}

\def\multlambindots{\pairlistdots{\lambda\varlangle\nonscript\,}
{\nonscript\,\varrangle.\;}{,\nonscript\:}\in}

%
%
%

\def\lambsub#1#2{\lambda{#1}_{#2}.\;}
\def\Lambop#1{\Lambda{#1}.\;}
\def\Deltop#1{\Delta{#1}.\;}


%

%
%
%
%
%
%

%
%
%
%

%
%
%
%
%
%

%
%
%

%
%

%
%

%
%

%
%

%
%

%

%
%

%

%
%
%
%
%

%
%
%
%
%

%
%
%
%
%

%
%
%
%
%

%

%

%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%

%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\def\multscript#1#2#3#4#5#6#7#8#9{{
\setbox\yybxA=\hbox{$\mathsurround=0pt\mathop{{#1}}$}%
\setbox\yybxB=\hbox{$\mathsurround=0pt#9{{#2}}$}%
\setbox\yybxC=\hbox{$\mathsurround=0pt#9{{#3}}$}%
\setbox\yybxD=\hbox{$\mathsurround=0pt#9{{#4}}$}%
\setbox\yybxE=\hbox{$\mathsurround=0pt#9{{#5}}$}%
\yydmA=\ht\yybxA%
\yydmB=\dp\yybxA%
\yydmC=\yydmA\advance\yydmC by #6%
\yydmD=\yydmB\advance\yydmD by #6%
\yydmE=\wd\yybxA%
\yydmF=\yydmE\advance\yydmF by 0pt%
\ht\yybxA=\yydmC\dp\yybxA=\yydmD%
%
\setbox\yybxF=\hbox{$\mathsurround=0pt#8\mathop{\box\yybxA}\limits
\ifdim\wd\yybxB=0pt\else\ifdim\wd\yybxB>\yydmF\else _{{#2}}\fi\fi
\ifdim\wd\yybxC=0pt\else\ifdim\wd\yybxC>\yydmF\else ^{{#3}}\fi\fi$}%
\yydmG=\ht\yybxF%
\yydmH=\dp\yybxF%
\yydmI=\wd\yybxF%
\ht\yybxF=\yydmA\dp\yybxF=\yydmB%
%
\setbox\yybxG=\hbox{$\mathsurround=0pt#8\mathop{\box\yybxF}\nolimits
\ifdim\wd\yybxD=0pt\else _{{#4}}\fi
\ifdim\wd\yybxE=0pt\else ^{{#5}}\fi
\vrule height\yydmC depth\yydmD width0pt$}%
\yydmA=\wd\yybxG%
\yydmB=\yydmE\advance\yydmB by -\yydmI\divide\yydmB by 2\relax
\advance\yydmB by #7\relax\ifdim\yydmB<0pt\yydmB=0pt\fi%
\yydmC=\yydmB \advance \yydmC by \yydmI \advance\yydmC by -\yydmA%
%
\setbox\yybxD=\hbox{$\mathsurround=0pt#8\mathop
{\kern\yydmB\box\yybxG\kern\yydmC}\limits
\ifdim\wd\yybxB=0pt\else\ifdim\wd\yybxB>\yydmF _{{#2}}\fi\fi
\ifdim\wd\yybxC=0pt\else\ifdim\wd\yybxC>\yydmF ^{{#3}}\fi\fi$}%
\yydmD=\yydmI\advance\yydmD by \wd\yybxD\divide\yydmD by -2\relax
\advance\yydmD by \yydmA\relax\ifdim\yydmD<0pt\yydmD=0pt\fi%
\box\yybxD\kern\yydmD\vrule height\yydmG depth\yydmH width0pt}}

%
%
%
%
%
%
%
%
%
%
%
%
%

\def\compscript#1#2#3#4#5#6#7#8#9{{
\setbox\yybxA=\hbox{$\mathsurround=0pt\mathop{{#1}}$}%
\setbox\yybxB=\hbox{$\mathsurround=0pt#9{{#2}}$}%
\setbox\yybxC=\hbox{$\mathsurround=0pt#9{{#3}}$}%
\setbox\yybxD=\hbox{$\mathsurround=0pt#9{{#4}}$}%
\setbox\yybxE=\hbox{$\mathsurround=0pt#9{{#5}}$}%
\yydmA=\ht\yybxA\advance\yydmA by #6%
\yydmB=\dp\yybxA\advance\yydmB by #6%
\yydmC=\wd\yybxA%
\yydmD=\wd\yybxE\advance\yydmD by -\wd\yybxD%
%
\setbox\yybxF=\hbox{$\mathsurround=0pt#8\mathop{\box\yybxA}\nolimits
\ifdim\wd\yybxD=0pt\else _{{#4}}\fi
\ifdim\wd\yybxE=0pt\else ^{{#5}}\fi$}%
\yydmE=\wd\yybxF\relax%
%
\ifdim\wd\yybxB=0pt\ifdim\wd\yybxC=0pt%
\setbox\yybxG=\box\yybxF%
\else%
\setbox\yybxG=\hbox{$\mathsurround=0pt#8\mathop{\box\yybxF
\ifdim\yydmD<0pt\kern\yydmD\else\fi}\nolimits ^{{#3}}$}%
\fi\else%
\ifdim\wd\yybxD=0pt\else\yydmF=\dp\yybxF
\advance\yydmF by 1pt\dp\yybxF=\yydmF\relax\fi
\ifdim\wd\yybxC=0pt%
\setbox\yybxG=\hbox{$\mathsurround=0pt#8\mathop{\box\yybxF
\ifdim\yydmD>0pt\kern-\yydmD\else\fi}\nolimits _{{#2}}$}%
\else%
\setbox\yybxG=\hbox{$\mathsurround=0pt#8\mathop{\box\yybxF
}\nolimits _{{#2}}^{{#3}}$}%
\fi\fi
\advance\yydmE by -\wd\yybxG%
\advance\yydmC by -\wd\yybxG\advance\yydmC by #7\relax%
\ifdim\yydmE<0pt\yydmE=0pt\else\fi\relax%
\ifdim\yydmC>\yydmE\yydmE=\yydmC\else\fi%
\kern #7\box\yybxG\kern\yydmE\vrule height\yydmA depth\yydmB width0pt}}

%
%
%
%
%
%
%
%
%

%
%
%
%
%

\def\prodms#1#2#3#4{\mathop{\mathchoice
{\multscript{\yylopstyle\oldprod}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\yylopstyle}{\scriptstyle}}
{\compscript{\textstyle\oldprod}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript{\scriptstyle\Pi}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript{\scriptscriptstyle\Pi}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\summs#1#2#3#4{\mathop{\mathchoice
{\multscript{\yylopstyle\oldsum}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\yylopstyle}{\scriptstyle}}
{\compscript{\textstyle\oldsum}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript{\scriptstyle\Sigma}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript{\scriptscriptstyle\Sigma}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\Lmms#1#2#3#4{\mathop{\mathchoice
{\multscript{\displaystyle{\rm Lm}}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\displaystyle}{\scriptstyle}}
{\compscript{\textstyle{\rm Lm}}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript{\scriptstyle{\rm Lm}}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript{\scriptscriptstyle{\rm Lm}}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\Colms#1#2#3#4{\mathop{\mathchoice
{\multscript{\displaystyle{\rm Col}}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\displaystyle}{\scriptstyle}}
{\compscript{\textstyle{\rm Col}}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript{\scriptstyle{\rm Col}}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript{\scriptscriptstyle{\rm Col}}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\Lubms#1#2#3#4{\mathop{\mathchoice
{\multscript{\yylopstyle\bigsqcup}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\yylopstyle}{\scriptstyle}}
{\compscript{\textstyle\bigsqcup}{#1}{#2}{#3}{#4}
{0pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\raise-0.19355ex\hbox{$\mathsurround=0pt{\textstyle\sqcup}$}}
{#1}{#2}{#3}{#4}{0pt}{0pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\raise-0.13548ex\hbox{$\mathsurround=0pt{\scriptstyle\sqcup}$}}
{#1}{#2}{#3}{#4}{0pt}{0pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\Glbms#1#2#3#4{\mathop{\mathchoice
{\ifnum\yylopstyleswitch=1\relax
\multscript{\kern0.25pt
\vrule height10.53pt depth3.25pt width0.7pt
\vrule height10.53pt depth-9.83pt width8.25pt
\vrule height10.53pt depth3.25pt width0.7pt
\vrule height11.0pt depth5.0pt width0pt\kern1.2111pt}
{#1}{#2}{#3}{#4}{0pt}{0pt}{\displaystyle}{\scriptstyle}
\else \multscript{\setbox\yybxB=\hbox{\kern0.25pt
\vrule height8.37pt depth1.2pt width0.7pt
\vrule height8.37pt depth-7.67pt width5.5pt
\vrule height8.37pt depth1.2pt width0.7pt\kern1.18333pt}
\ht\yybxB=8.0pt\dp\yybxB=2.0pt\relax\box\yybxB}
{#1}{#2}{#3}{#4}{0pt}{0pt}{\textstyle}{\scriptstyle}\fi}
{\compscript{\setbox\yybxB=\hbox{\kern0.25pt
\vrule height8.37pt depth1.2pt width0.7pt
\vrule height8.37pt depth-7.67pt width5.5pt
\vrule height8.37pt depth1.2pt width0.7pt\kern1.18333pt}
\ht\yybxB=8.0pt\dp\yybxB=2.0pt\relax\box\yybxB}
{#1}{#2}{#3}{#4}{0pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\raise-1pt\hbox{$\mathsurround=0pt{\textstyle\sqcap}$}}
{#1}{#2}{#3}{#4}{0pt}{0pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\raise-0.7pt\hbox{$\mathsurround=0pt{\scriptstyle\sqcap}$}}
{#1}{#2}{#3}{#4}{0pt}{0pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}


%

%
%
%

%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%

\def\encircle#1#2#3#4{\setlength{\unitlength}{0.1pt}
\begin{picture}(0,0)
\put(#1,#2){\circle{#3}}
\end{picture}
{#4}}

%
%
%
%
%

\def\cirprodmsnorm#1#2#3#4{\mathop{\mathchoice
{\ifnum\yylopstyleswitch=1\relax
\multscript
{\kern3.5pt\encircle{59}{34}{200}{\displaystyle\oldprod}\kern3.5pt}
{#1}{#2}{#3}{#4}{2.5pt}{0.5pt}{\displaystyle}{\scriptstyle}
\else \multscript
{\kern2.5pt\encircle{42}{34}{140}{\textstyle\oldprod}\kern2.5pt}
{#1}{#2}{#3}{#4}{2.0pt}{0pt}{\textstyle}{\scriptstyle}\fi}
{\compscript
{\kern2.5pt\encircle{42}{34}{140}{\textstyle\oldprod}\kern2.5pt}
{#1}{#2}{#3}{#4}{1.5pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1.75pt\encircle{31}{27}{90}{\scriptstyle\Pi}\kern1.75pt}
{#1}{#2}{#3}{#4}{1pt}{0.5pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\kern1pt\encircle{23}{20}{70}{\scriptscriptstyle\Pi}\kern1pt}
{#1}{#2}{#3}{#4}{0.5pt}{0.25pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\cirsummsnorm#1#2#3#4{\mathop{\mathchoice
{\ifnum\yylopstyleswitch=1\relax
\multscript
{\kern2.5pt\encircle{65}{33}{200}{\displaystyle\oldsum}\kern2.5pt}
{#1}{#2}{#3}{#4}{2.5pt}{1.0pt}{\displaystyle}{\scriptstyle}
\else \multscript
{\kern2.5pt\encircle{47}{34}{150}{\textstyle\oldsum}\kern2.5pt}
{#1}{#2}{#3}{#4}{2.75pt}{0pt}{\textstyle}{\scriptstyle}\fi}
{\compscript
{\kern2.5pt\encircle{47}{34}{150}{\textstyle\oldsum}\kern2.5pt}
{#1}{#2}{#3}{#4}{2.25pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1.25pt\encircle{27}{28}{80}{\scriptstyle\Sigma}\kern1.25pt}
{#1}{#2}{#3}{#4}{1pt}{0.5pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\kern1.25pt\encircle{25}{19}{70}{\scriptscriptstyle\Sigma}\kern1.25pt}
{#1}{#2}{#3}{#4}{0.5pt}{0.5pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\cirLmmsnorm#1#2#3#4{\mathop{\mathchoice
{\multscript
{\kern2pt\encircle{87}{37}{200}{\textstyle{\rm Lm}}\kern2pt}
{#1}{#2}{#3}{#4}{6pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern2pt\encircle{87}{37}{200}{\textstyle{\rm Lm}}\kern2pt}
{#1}{#2}{#3}{#4}{6pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1.5pt\encircle{61}{27}{140}{\scriptstyle{\rm Lm}}\kern1.5pt}
{#1}{#2}{#3}{#4}{3.5pt}{0.5pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\kern1pt\encircle{51}{20}{120}{\scriptscriptstyle{\rm Lm}}\kern1pt}
{#1}{#2}{#3}{#4}{3pt}{0.3pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\cirColmsnorm#1#2#3#4{\mathop{\mathchoice
{\multscript
{\kern2pt\encircle{93}{35}{200}{\textstyle{\rm Col}}\kern2pt}
{#1}{#2}{#3}{#4}{6.25pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern2pt\encircle{93}{35}{200}{\textstyle{\rm Col}}\kern2pt}
{#1}{#2}{#3}{#4}{6.25pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1.5pt\encircle{65}{24}{140}{\scriptstyle{\rm Col}}\kern1.5pt}
{#1}{#2}{#3}{#4}{4pt}{0.5pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\kern1.25pt\encircle{57}{21}{130}{\scriptscriptstyle{\rm Col}}\kern1.25pt}
{#1}{#2}{#3}{#4}{3.5pt}{0.5pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

%
%
%
%

\def\cirprodmsshrunk#1#2#3#4{\mathop{\mathchoice
{\ifnum\yylopstyleswitch=1\relax
\multscript
{\kern2.25pt\raise0.2pt\hbox{$\mathsurround=0pt\encircle{43}{35}{150}
{\textstyle\oldprod}$}
\vrule height11.0pt depth5.0pt width0pt\kern2.25pt}
{#1}{#2}{#3}{#4}{0pt}{1.5pt}{\displaystyle}{\scriptstyle}
\else \multscript
{\kern1.75pt\raise-0.6pt\hbox{$\mathsurround=0pt\encircle{42}{41}{120}
{\textstyle\Pi}$}
\vrule height8.0pt depth2.0pt width0pt\kern1.75pt}
{#1}{#2}{#3}{#4}{1.0pt}{0.5pt}{\textstyle}{\scriptstyle}\fi}
{\compscript
{\kern1.75pt\raise-0.6pt\hbox{$\mathsurround=0pt\encircle{42}{41}{120}
{\textstyle\Pi}$}
\vrule height8.0pt depth2.0pt width0pt\kern1.75pt}
{#1}{#2}{#3}{#4}{0.5pt}{0.5pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1pt\raise0.6875pt\hbox{$\mathsurround=0pt\encircle{23}{20}{70}
{\scriptscriptstyle\Pi}$}
\vrule height5.47221pt depth0pt width0pt\kern1pt}
{#1}{#2}{#3}{#4}{0.5pt}{0.5pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\kern1pt\encircle{23}{20}{70}{\scriptscriptstyle\Pi}\kern1pt}
{#1}{#2}{#3}{#4}{0.5pt}{0.25pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\cirsummsshrunk#1#2#3#4{\mathop{\mathchoice
{\ifnum\yylopstyleswitch=1\relax
\multscript
{\kern1.75pt\raise0.2pt\hbox{$\mathsurround=0pt\encircle{47}{34}{150}
{\textstyle\oldsum}$}
\vrule height11.0pt depth5.0pt width0pt\kern1.75pt}
{#1}{#2}{#3}{#4}{0pt}{1.5pt}{\displaystyle}{\scriptstyle}
\else \multscript
{\kern2.0pt\raise-0.6pt\hbox{$\mathsurround=0pt\encircle{38}{41}{120}
{\textstyle\Sigma}$}
\vrule height8.0pt depth2.0pt width0pt\kern2.0pt}
{#1}{#2}{#3}{#4}{1.25pt}{0.5pt}{\textstyle}{\scriptstyle}\fi}
{\compscript
{\kern2.0pt\raise-0.6pt\hbox{$\mathsurround=0pt\encircle{38}{41}{120}
{\textstyle\Sigma}$}
\vrule height8.0pt depth2.0pt width0pt\kern2.0pt}
{#1}{#2}{#3}{#4}{0.75pt}{0.5pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1.5pt\raise0.6875pt\hbox{$\mathsurround=0pt\encircle{25}{19}{70}
{\scriptscriptstyle\Sigma}$}
\vrule height5.47221pt depth0pt width0pt\kern1.5pt}
{#1}{#2}{#3}{#4}{0.5pt}{0.3pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\kern1.25pt\encircle{25}{19}{70}{\scriptscriptstyle\Sigma}\kern1.25pt}
{#1}{#2}{#3}{#4}{0.5pt}{0.5pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\cirLmmsshrunk#1#2#3#4{\mathop{\mathchoice
{\multscript
{\kern1.5pt\raise1.36pt\hbox{$\mathsurround=0pt\encircle{61}{27}{140}
{\scriptstyle{\rm Lm}}$}
\vrule height8.2pt depth0pt width0pt\kern1.5pt}
{#1}{#2}{#3}{#4}{3pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1.5pt\raise1.36pt\hbox{$\mathsurround=0pt\encircle{61}{27}{140}
{\scriptstyle{\rm Lm}}$}
\vrule height8.2pt depth0pt width0pt\kern1.5pt}
{#1}{#2}{#3}{#4}{3pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1.25pt\raise0.90pt\hbox{$\mathsurround=0pt\encircle{51}{20}{120}
{\scriptscriptstyle{\rm Lm}}$}
\vrule height5.47221pt depth0pt width0pt\kern1.25pt}
{#1}{#2}{#3}{#4}{2.5pt}{0.5pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\kern1pt\encircle{51}{20}{120}{\scriptscriptstyle{\rm Lm}}\kern1pt}
{#1}{#2}{#3}{#4}{3pt}{0.3pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

\def\cirColmsshrunk#1#2#3#4{\mathop{\mathchoice
{\multscript
{\kern2pt\raise1.00pt\hbox{$\mathsurround=0pt\encircle{66}{26}{150}
{\scriptstyle{\rm Col}}$}
\vrule height8.33333pt depth0pt width0pt\kern2pt}
{#1}{#2}{#3}{#4}{3.5pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern2pt\raise1.00pt\hbox{$\mathsurround=0pt\encircle{66}{26}{150}
{\scriptstyle{\rm Col}}$}
\vrule height8.33333pt depth0pt width0pt\kern2pt}
{#1}{#2}{#3}{#4}{3.5pt}{0pt}{\textstyle}{\scriptstyle}}
{\compscript
{\kern1.5pt\raise0.68pt\hbox{$\mathsurround=0pt\encircle{57}{21}{130}
{\scriptscriptstyle{\rm Col}}$}
\vrule height5.55556pt depth0pt width0pt\kern1.5pt}
{#1}{#2}{#3}{#4}{2.75pt}{0.75pt}{\scriptstyle}{\scriptscriptstyle}}
{\compscript
{\kern1.25pt\encircle{57}{21}{130}{\scriptscriptstyle{\rm Col}}\kern1.25pt}
{#1}{#2}{#3}{#4}{3.5pt}{0.5pt}{\scriptscriptstyle}{\scriptscriptstyle}}}}

%
%
%
%
%
%

%
%

\def\largecircleops{
\let\cirprodms=\cirprodmsnorm
\let\cirsumms=\cirsummsnorm
\let\cirLmms=\cirLmmsnorm
\let\cirColms=\cirColmsnorm}

\def\smallcircleops{
\let\cirprodms=\cirprodmsshrunk
\let\cirsumms=\cirsummsshrunk
\let\cirLmms=\cirLmmsshrunk
\let\cirColms=\cirColmsshrunk}

\largecircleops



==> diagmac.tex <==
%

%
%
%
%

%

%
\def\diagramunit{1pt}%
%
\def\centerheight{3pt}
\def\edgeheaddisp{4pt}
\def\circleheaddisp{2pt}
\def\diameterlist{1pt,2pt,3pt,4pt,5pt,6pt,7pt,8pt,9pt,10pt,11pt,%
12pt,13pt,14pt,15pt,16pt,20pt,24pt,28pt,32pt,36pt,40pt,}
%

%
%
\newdimen\texpr\newdimen\bexpr\newdimen\lexpr\newdimen\rexpr%
\newdimen\xcenter\newdimen\ycenter%
\newcount\xslope\newcount\yslope%
\newdimen\xstart\newdimen\ystart%
\newdimen\xend\newdimen\yend%
\newdimen\dcircle%
\newdimen\xcircle\newdimen\ycircle%
\newcount\zzisedge%
\newcount\zziscircle%
\newbox\zzdiagbox%
\newdimen\zztotlwidth\newdimen\zztotrwidth%
\newdimen\zztotheight\newdimen\zztotdepth%

%
%
\newdimen\zzglobaltotlwidth\newdimen\zzglobaltotrwidth
\newdimen\zzglobaltotheight\newdimen\zzglobaltotdepth
\newdimen\zzglobalxcenter\newdimen\zzglobalycenter
\newcount\zzglobalcnA

%
\newdimen\zzdmA\newdimen\zzdmB\newdimen\zzdmC\newdimen\zzdmD\newdimen\zzdmE
\newdimen\zzdmF\newdimen\zzdmG\newdimen\zzdmH\newdimen\zzdmI
\newcount\zzcnA\newcount\zzcnB\newcount\zzcnC
\newcount\zzcnD\newcount\zzcnE\newcount\zzcnF
\newcount\zzcnG\newcount\zzcnH\newcount\zzcnI

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%

\def\diagram#1{{\setbox\zzdiagbox=\hbox{$\mathsurround=0pt
\zztotlwidth=0pt\zztotrwidth=0pt\def\zzvertexlist{\end}\zzisedge=0\relax
#1\relax\kern\zztotrwidth\global\zzglobaltotlwidth=\zztotlwidth $}
\kern-\zzglobaltotlwidth\box\zzdiagbox}}

%
%
%
%
%
%
%

\def\zzsetupbox#1#2{\setbox\zzdiagbox=\hbox{$\mathsurround=0pt
\setbox\zzdiagbox=\hbox{$\mathsurround=0pt{{#1}}$}
\texpr=\ht\zzdiagbox\bexpr=-\dp\zzdiagbox\rexpr=\wd\zzdiagbox\lexpr=0pt
\xcenter=\rexpr\divide\xcenter by 2\ycenter=\centerheight
\zztotlwidth=0pt\zztotrwidth=\rexpr\def\zzshadow{\zznoshadow0pt,0pt:;}
\zziscircle=0
\box\zzdiagbox\kern-\rexpr
#2\relax
\global\zzglobalxcenter=\xcenter\global\zzglobalycenter=\ycenter
\global\zzglobaltotlwidth=\zztotlwidth\kern\zztotrwidth
\global\let\zzglobalshadow=\zzshadow
$}}

%

\def\zznoshadow#1,#2:;{\errmessage{ATTEMPT TO OUTLINE OR ABUT AN EXPRESSION
WITH NO SHADOW}}

%
%

\def\leftghost#1{\setbox\zzdiagbox=\hbox{$\mathsurround=0pt{{#1}}$}
\xcenter=\wd\zzdiagbox\divide\xcenter by 2\advance\xcenter by \lexpr}

\def\rightghost#1{\setbox\zzdiagbox=\hbox{$\mathsurround=0pt{{#1}}$}
\xcenter=\wd\zzdiagbox\divide\xcenter by -2\advance\xcenter by \rexpr}

%
%
%

\def\zzissue{\advance\zzdmA by -\zzglobalxcenter
\advance\zzdmB by -\zzglobalycenter
\zzdmC=\zzdmA\advance\zzdmC by \wd\zzdiagbox
\zzdmD=\zzdmA\advance\zzdmD by \zzglobaltotlwidth
\zzrecordwidth\zzdmD\zzdmC
\kern\zzdmA\raise\zzdmB\box\zzdiagbox\kern-\zzdmC}

%
%
%

\def\zzrecordwidth#1#2{\relax\ifdim#1<\zztotlwidth\relax\zztotlwidth=#1\fi
\ifdim\zztotrwidth<#2\relax\zztotrwidth=#2\fi}

%
%
%

\def\zzrecordheight#1#2{\relax\ifdim\zztotheight<#1\relax\zztotheight=#1\fi
\ifdim#2<\zztotdepth\relax\zztotdepth=#2\fi}

%
%
%
%

\def\placed#1#2#3#4{\zzsetupbox{#3}{#4}\zzdmA=#1\zzdmB=#2\zzissue}

\def\place#1,#2:#3#4{\zzsetupbox{#3}{#4}\zzmultdiagramunit\zzdmA{#1}
\zzmultdiagramunit\zzdmB{#2}\zzissue}

%

\def\zzmultdiagramunit#1#2{#1=\diagramunit\multiply#1 by #2\relax}

%
%
%
%
%
%

\def\vertex#1,#2:#3#4{\place{#1},{#2}:{#3}{#4}\zzcnA=#1\zzcnB=#2\relax
\expandafter\zzconsvertexlist\zzglobalshadow}

\def\zzconsvertexlist#1#2,#3:#4;{\def\zztesta{#1}\def\zztestb{\zznoshadow}
\ifx\zztesta\zztestb\else
\advance\zzdmA by #2\advance\zzdmB by #3\relax
\edef\zzvertexitem{\the\zzcnA,\the\zzcnB:\noexpand #1\the\zzdmA,\the\zzdmB:#4;}
\expandafter\zzconsvertexlista\zzvertexlist\fi}

\def\zzconsvertexlista{\expandafter\zzconsvertexlistb\zzvertexitem}

\def\zzconsvertexlistb#1\end{\def\zzvertexlist{#1\end}}

%
%
%
%
%
%
%
%
%
%
%
%

\def\rect{\zzdmC=\rexpr\advance\zzdmC by -\lexpr
\zzdmD=\texpr\advance\zzdmD by -\bexpr
\zzisnegside{\zzdmC}{RECT}\zzisnegside{\zzdmD}{RECT}
\edef\zzshadow{\noexpand\zzprocrect
\the\lexpr,\the\texpr:\the\zzdmC,\the\zzdmD;}}

\def\zzprocrect#1,#2:#3,#4;{\zzprocpoly
{#1}{#2}{10{#3}0{-1}{#4}{-1}0{#3}01{#4}}}

\def\zzisnegside#1#2{\relax\ifdim#1<0pt\errmessage
{#2 WITH NEGATIVE SIDE}\fi}

\def\hexagon{\zzdmC=\rexpr\advance\zzdmC by -\lexpr
\zzdmD=\texpr\advance\zzdmD by -\bexpr\divide\zzdmD by 4
\zzisnegside{\zzdmC}{HEXAGON}\zzisnegside{\zzdmD}{HEXAGON}
\edef\zzshadow{\noexpand\zzprochexagon
\the\lexpr,\the\texpr:\the\zzdmC,\the\zzdmD;}}

\def\zzprochexagon#1,#2:#3,#4;{\zzprocpoly{#1}{#2}
{10{#3}1{-2}{#4}{-1}{-2}{#4}{-1}0{#3}{-1}2{#4}12{#4}}}

\def\octagon#1{\zzdmC=#1\zzdmD=\zzdmC\multiply\zzdmD by -2\zzdmE=\zzdmD
\advance\zzdmD by \rexpr\advance\zzdmD by -\lexpr
\advance\zzdmE by \texpr\advance\zzdmE by -\bexpr
\zzdmF=\lexpr\advance\zzdmF by \zzdmC
\zzisnegside{\zzdmC}{OCTAGON}\zzisnegside{\zzdmD}{OCTAGON}
\zzisnegside{\zzdmE}{OCTAGON}
\edef\zzshadow{\noexpand\zzprococtagon
\the\zzdmF,\the\texpr:\the\zzdmC,\the\zzdmD,\the\zzdmE;}}

\def\zzprococtagon#1,#2:#3,#4,#5;{\zzprocpoly{#1}{#2}
{10{#4}1{-1}{#3}0{-1}{#5}{-1}{-1}{#3}{-1}0{#4}{-1}1{#3}01{#5}11{#3}}}

\def\diamond{\zzdmC=\texpr\advance\zzdmC by -\bexpr
\advance\zzdmC by \rexpr\advance\zzdmC by -\lexpr\divide\zzdmC by 2
\zzdmD=\lexpr\advance\zzdmD by \rexpr\divide\zzdmD by 2
\zzdmE=\texpr\advance\zzdmE by \bexpr\divide\zzdmE by 2\advance\zzdmE by \zzdmC
\zzisnegside{\zzdmC}{DIAMOND}
\edef\zzshadow{\noexpand\zzprocdiamond
\the\zzdmD,\the\zzdmE:\the\zzdmC;}}

\def\zzprocdiamond#1,#2:#3;{\zzprocpoly{#1}{#2}
{1{-1}{#3}{-1}{-1}{#3}{-1}1{#3}11{#3}}}

\def\rorect#1#2#3{\zzcheckposdimen{#1}{FIRST}{RORECT}
\zzcheckbool{#2}{SECOND}{RORECT}\zzcheckbool{#3}{THIRD}{RORECT}
\zzdmD=\rexpr\advance\zzdmD by -\lexpr\zzdmE=\texpr\advance\zzdmE by -\bexpr
\zzdmC=#1\relax
\ifnum#2=1\relax\ifdim\zzdmD>\zzdmC\relax\zzdmC=\zzdmD\fi\fi
\ifnum#3=1\relax\ifdim\zzdmE>\zzdmC\relax\zzdmC=\zzdmE\fi\fi
\expandafter\zzsearchdiameterlist\diameterlist\end\zzdmC=\zzdmF\relax
\ifdim\zzdmC>\zzdmD\relax\zzdmD=\zzdmC\fi
\ifdim\zzdmC>\zzdmE\relax\zzdmE=\zzdmC\fi
\zzdmF=\lexpr\advance\zzdmF by \rexpr\divide\zzdmF by 2
\zzdmG=\bexpr\advance\zzdmG by \texpr\divide\zzdmG by 2
\edef\zzshadow{\noexpand\zzprocrorect
\the\zzdmF,\the\zzdmG:\the\zzdmC,\the\zzdmD,\the\zzdmE;}}

\def\zzsearchdiameterlist#1{\def\zztesta{#1}\def\zztestb{\end}
\ifx\zztesta\zztestb\let\zznext=\zzsearchdiameterlista
\else\let\zznext=\zzsearchdiameterlistb\fi\zznext #1}

\def\zzsearchdiameterlista#1\end{}

\def\zzsearchdiameterlistb#1,{\zzdmF=#1\relax
\ifdim\zzdmF<\zzdmC\relax\let\zznext=\zzsearchdiameterlist
\else\let\zznext=\zzsearchdiameterlista\fi\zznext}

%
%

\def\outline{\def\zzprocpoly{\zzoutlinepoly}
\def\zzprocrorect{\zzoutlinerorect}\zzshadow}

%

\def\zzmakepicture#1{{\setlength{\unitlength}{1sp}\begin{picture}(0,0)
#1\relax
\global\zzglobaltotlwidth=\zztotlwidth\global\zzglobaltotrwidth=\zztotrwidth
\global\zzglobaltotheight=\zztotheight\global\zzglobaltotdepth=\zztotdepth
\end{picture}\vrule height\zzglobaltotheight depth-\zzglobaltotdepth width0pt}
\zztotlwidth=\zzglobaltotlwidth\zztotrwidth=\zzglobaltotrwidth}

\def\zzoutlinepoly#1#2#3{\zzmakepicture{\zzdmA=#1\zzdmB=#2\relax
\zztotheight=\zzdmB\zztotdepth=\zzdmB\zzoutlinepolya #3\end}}

\def\zzoutlinepolya#1{\def\zztesta{#1}\def\zztestb{\end}
\ifx\zztesta\zztestb\let\zznext=\zzoutlinepolyb
\else\let\zznext=\zzoutlinepolyc\fi\zznext {#1}}

\def\zzoutlinepolyb#1{}

\def\zzoutlinepolyc#1#2#3{\zzrecordwidth\zzdmA\zzdmA\zzrecordheight\zzdmB\zzdmB
\zzdmE=#3\multiply\zzdmE by #1\zzdmF=#3\multiply\zzdmF by #2\relax
\zzcnA=\zzdmA\zzcnB=\zzdmB\relax
\ifnum #1=0\relax\zzcnC=\zzdmF\else\zzcnC=\zzdmE\fi
\ifnum\zzcnC<0\relax\zzcnC=-\zzcnC\fi
\put(\zzcnA,\zzcnB){\line(#1,#2){\zzcnC}}
\advance\zzdmA by \zzdmE\advance\zzdmB by \zzdmF
\zzoutlinepolya}

\def\zzoutlinerorect#1,#2:#3,#4,#5;{\zzmakepicture{
\zzdmA=#1\zzdmB=#2\zzdmC=#3\zzdmD=#4\zzdmE=#5
\zzcnA=\zzdmA\zzcnB=\zzdmB\zzcnC=\zzdmC\zzcnD=\zzdmD\zzcnE=\zzdmE
\ifnum\zzcnD=\zzcnC\relax\put(\zzcnA,\zzcnB){\oval(\zzcnD,\zzcnE)}
\else\ifnum\zzcnE=\zzcnC\relax\put(\zzcnA,\zzcnB){\oval(\zzcnD,\zzcnE)}
\else\advance\zzcnE by -\zzcnC
\zzcnF=\zzcnE\divide\zzcnF by 2\advance\zzcnF by \zzcnB
\put(\zzcnA,\zzcnF){\oval(\zzcnD,\zzcnC)[t]}
\advance\zzcnF by -\zzcnE
\put(\zzcnA,\zzcnF){\oval(\zzcnD,\zzcnC)[b]}
\zzcnC=\zzcnD\divide\zzcnC by 2\advance\zzcnA by \zzcnC
\put(\zzcnA,\zzcnF){\line(0,1){\zzcnE}}
\advance\zzcnA by -\zzcnD
\put(\zzcnA,\zzcnF){\line(0,1){\zzcnE}}\fi\fi
\zztotheight=\zzdmE\divide\zztotheight by 2\advance\zztotheight by \zzdmB
\zztotdepth=\zztotheight\advance\zztotdepth by -\zzdmE
\zzdmC=\zzdmD\divide\zzdmC by -2\advance\zzdmC by \zzdmA
\advance\zzdmD by \zzdmC\zzrecordwidth\zzdmC\zzdmD}}

%

\def\border#1#2{\advance\texpr by #2\advance\bexpr by -#2
\advance\lexpr by -#1\advance\rexpr by #1}

\def\borderto#1#2{\zzdmA=\rexpr\advance\zzdmA by -\lexpr\relax
\ifdim#1>\zzdmA\relax\advance\zzdmA by -#1\divide\zzdmA by 2
\advance\rexpr by -\zzdmA\advance\lexpr by \zzdmA\fi
\zzdmA=\texpr\advance\zzdmA by -\bexpr\relax
\ifdim#2>\zzdmA\relax\advance\zzdmA by -#2\divide\zzdmA by 2
\advance\texpr by -\zzdmA\advance\bexpr by \zzdmA\fi}

\def\symmetrize{\zzdmA=\texpr\advance\zzdmA by -\ycenter
\zzdmB=\ycenter\advance\zzdmB by -\bexpr\relax
\ifdim\zzdmA<\zzdmB\relax\zzdmA=\zzdmB\fi
\texpr=\ycenter\advance\texpr by \zzdmA
\bexpr=\ycenter\advance\bexpr by -\zzdmA}

%
%
%
%
%
%
%

\def\setedge#1,#2,#3,#4:{\zzcnA=#1\zzcnB=#2
\zzmultdiagramunit\xstart\zzcnA\zzmultdiagramunit\ystart\zzcnB
\expandafter\zzsearchvertexlist\zzvertexlist
\let\zzstartshadow=\zzshadow
\zzcnA=#3\zzcnB=#4
\zzmultdiagramunit\xend\zzcnA\zzmultdiagramunit\yend\zzcnB
\expandafter\zzsearchvertexlist\zzvertexlist
\let\zzendshadow=\zzshadow
\xslope=#3\advance\xslope by -#1\relax
\yslope=#4\advance\yslope by -#2\relax
\zzreduceterms\xslope\yslope{START AND END OF EDGE ARE BOTH THE SAME}
\xslope=\zzcnC\yslope=\zzcnD\zzisedge=1}

%
%
%

\def\zzreduceterms#1#2#3{{
\ifnum#1<0\relax\zzcnA=-#1\else\zzcnA=#1\fi
\ifnum#2<0\relax\zzcnB=-#2\else\zzcnB=#2\fi
\loop\ifnum\zzcnB>0\relax
\zzcnC=\zzcnA\divide\zzcnC by \zzcnB\multiply\zzcnC by -\zzcnB
\advance\zzcnC by \zzcnA\zzcnA=\zzcnB\zzcnB=\zzcnC
\repeat\relax
\ifnum\zzcnA=0\errmessage{#3}\fi
\global\zzglobalcnA=\zzcnA}
\zzcnC=#1\divide\zzcnC by \zzglobalcnA\zzcnD=#2\divide\zzcnD by \zzglobalcnA}

%
%
%
%

\def\zzsearchvertexlist#1{\def\zztesta{#1}\def\zztestb{\end}
\ifx\zztesta\zztestb\def\zzshadow{\zzdmE=\zzdmA\zzdmF=\zzdmB}
\let\zznext=\zzsearchvertexlista
\else\let\zznext=\zzsearchvertexlistb\fi\zznext #1}

\def\zzsearchvertexlista#1\end{}

\def\zzsearchvertexlistb#1,#2:#3;{\relax
\ifnum\zzcnA=#1\relax\ifnum\zzcnB=#2\relax
\def\zzshadow{#3;}\let\zznext=\zzsearchvertexlista
\else\let\zznext=\zzsearchvertexlist\fi
\else\let\zznext=\zzsearchvertexlist\fi\zznext}

%
%

\def\shadeedge{\zzcheckedge{SHADE}
\def\zzprocpoly{\zzcastpoly}\def\zzprocrorect{\zzprocrorecta}
\zzdmA=\xstart\zzdmB=\ystart\zzcnA=\xslope\zzcnB=\yslope
\zzstartshadow\xstart=\zzdmE\ystart=\zzdmF
\zzdmA=\xend\zzdmB=\yend\zzcnA=-\xslope\zzcnB=-\yslope
\zzendshadow\xend=\zzdmE\yend=\zzdmF}

\def\zzcheckedge#1{\relax\ifnum\zzisedge=0\relax\errmessage
{ATTEMPT TO #1 NONEXISTENT EDGE}\fi}

%
%
%

\def\zzprocrorecta#1,#2:#3,#4,#5;{\zzdmC=#3
\multiply\zzdmC by 53\divide\zzdmC by 181
\zzdmD=\zzdmC\multiply\zzdmD by -2\zzdmE=\zzdmD
\advance\zzdmD by #4\advance\zzdmE by #5
\zzdmF=#4\divide\zzdmF by -2\advance\zzdmF by #1\advance\zzdmF by \zzdmC
\zzdmG=#5\divide\zzdmG by 2\advance\zzdmG by #2
\edef\zzlocalshadow{\noexpand\zzprococtagon
\the\zzdmF,\the\zzdmG:\the\zzdmC,\the\zzdmD,\the\zzdmE;}
\zzlocalshadow}

%
%
%
%
%
%
%

\def\zzcastpoly#1#2#3{\zzdmC=#1\zzdmD=#2\zzcnC=0
\zzcastpolya #3\end}

\def\zzcastpolya#1{\def\zztesta{#1}\def\zztestb{\end}
\ifx\zztesta\zztestb\let\zznext=\zzcastpolyg
\else\let\zznext=\zzcastpolyc\fi\zznext {#1}}

\def\zzcastpolyb#1\end{\zzcnC=\zzcnA\multiply\zzcnC by \zzcnA
\zzcnD=\zzcnB\multiply\zzcnD by \zzcnB\advance\zzcnC by \zzcnD
\zzdmE=\zzdmC\advance\zzdmE by -\zzdmA\multiply\zzdmE by \zzcnA
\zzdmF=\zzdmD\advance\zzdmF by -\zzdmB\multiply\zzdmF by \zzcnB
\advance\zzdmE by \zzdmF\divide\zzdmE by \zzcnC\zzdmF=\zzdmE
\multiply\zzdmE by \zzcnA\advance\zzdmE by \zzdmA
\multiply\zzdmF by \zzcnB\advance\zzdmF by \zzdmB}


\def\zzcastpolyc#1#2#3{\zzcnD=\zzcnB\multiply\zzcnD by #1\relax
\zzcnE=\zzcnA\multiply\zzcnE by #2\relax\advance\zzcnD by -\zzcnE\relax
\ifnum\zzcnD>0\relax
\ifnum\zzcnC=2\zzcastpolyd{#1}{#2}{#3}\let\zznext=\zzcastpolya\else
\zzdmE=\zzdmA\advance\zzdmE by -\zzdmC\multiply\zzdmE by \zzcnB
\zzdmF=\zzdmB\advance\zzdmF by -\zzdmD\multiply\zzdmF by \zzcnA
\advance\zzdmE by -\zzdmF\divide\zzdmE by \zzcnD\relax
\ifdim\zzdmE>#3\relax\zzcnC=3\zzcastpolyd{#1}{#2}{#3}\let\zznext=\zzcastpolya
\else\ifnum\zzcnC=3\zzcastpolyf{#1}{#2}\let\zznext=\zzcastpolye\else
\ifdim\zzdmE<0pt\relax
\ifnum\zzcnC=1\let\zznext=\zzcastpolyb\else
\zzcnC=2\zzcastpolyd{#1}{#2}{#3}\let\zznext=\zzcastpolya\fi
\else\zzcastpolyf{#1}{#2}\let\zznext=\zzcastpolye\fi\fi\fi\fi
\else\ifnum\zzcnC=3\let\zznext=\zzcastpolyb
\else\zzcnC=1\zzcastpolyd{#1}{#2}{#3}\let\zznext=\zzcastpolya\fi\fi
\zznext}

\def\zzcastpolyd#1#2#3{
\zzdmE=#3\multiply\zzdmE by #1\advance\zzdmC by \zzdmE
\zzdmE=#3\multiply\zzdmE by #2\advance\zzdmD by \zzdmE}

\def\zzcastpolye#1\end{}

\def\zzcastpolyf#1#2{\zzdmF=\zzdmE
\multiply\zzdmE by #1\relax\advance\zzdmE by \zzdmC
\multiply\zzdmF by #2\relax\advance\zzdmF by \zzdmD}

\def\zzcastpolyg#1{\zzcastpolyb\end}

%
%
%

\def\shiftedge#1{\zzcheckedge{SHIFT}
\zzdistance\xslope\yslope
\zzdmA=#1\multiply\zzdmA by 100\divide\zzdmA by \zzglobalcnA\zzdmB=\zzdmA
\multiply\zzdmA by -\yslope\multiply\zzdmB by \xslope
\advance\xstart by \zzdmA \advance\xend by \zzdmA
\advance\ystart by \zzdmB \advance\yend by \zzdmB}

%
%

\def\zzsqroot#1{{\zzcnA=#1
%
\zzcnC=0\zzcnD=1
\loop\zzcnE=\zzcnA\divide\zzcnE by \zzcnD\advance\zzcnE by 1
\relax\ifnum\zzcnD<\zzcnE\relax
\advance \zzcnC by 1\multiply\zzcnD by 2
\repeat
\zzcnB=0
\loop\ifnum\zzcnC>0\relax
\advance\zzcnC by -1\divide\zzcnD by 2
\zzcnE=\zzcnB\advance\zzcnE by \zzcnD\multiply\zzcnE by \zzcnE\relax
\ifnum\zzcnA<\zzcnE\relax\else\advance\zzcnB by \zzcnD\fi
\repeat
\global\zzglobalcnA=\zzcnB}}

%
%

\def\zzdistance#1#2{{\zzcnA=#1\multiply\zzcnA by \zzcnA
\zzcnB=#2\multiply\zzcnB by \zzcnB
\advance\zzcnA by \zzcnB\multiply\zzcnA by 10000
\zzsqroot\zzcnA}}

%
%

\def\drawdashedge#1#2#3#4{\zzcnA=1\zzdmA=#1\zzdmB=#2
\zzcheckposdimen\zzdmA{FIRST}{DRAWDASHEDGE}
\zzcheckposdimen\zzdmB{SECOND}{DRAWDASHEDGE}
\zzchecknonnegnum{#3}{THIRD}{DRAWDASHEDGE}
\zzchecknonnegnum{#4}{FOURTH}{DRAWDASHEDGE}
\zzcnI=#3\relax\advance\zzcnI by #4\relax
\ifnum\zzcnI>0\else\errmessage
{SUM OF THIRD AND FOURTH PARAMETERS OF DRAWDASHEDGE MUST BE POSITIVE}\fi
\advance\zzdmB by \zzdmA
\zzdrawedge{\advance\zzcnC by -\zzcnD
\zzcnG=\zzcnC\divide\zzcnG by \zzcnE\relax
\ifnum\zzcnG>0\relax
\zzcnH=\zzcnG\multiply\zzcnH by \zzcnE\advance\zzcnC by -\zzcnH
\zzcnH=\zzcnI\multiply\zzcnH by \zzcnG
\advance\zzcnH by #3\divide\zzcnC by \zzcnH
\zzcnH=#3\multiply\zzcnH by \zzcnC\advance\zzcnD by \zzcnH
\multiply\zzcnC by \zzcnI\advance\zzcnE by \zzcnC
\else\advance\zzcnD by \zzcnC\fi}
{\line(\xslope,\yslope){\zzcnD}}}

\def\zzcheckposdimen#1#2#3{\relax\ifdim#1>0pt\else\errmessage{
#2 PARAMETER OF #3 MUST BE POSITIVE}\fi}

\def\zzchecknonnegnum#1#2#3{\relax\ifnum#1<0\relax\errmessage{
#2 PARAMETER OF #3 MUST BE NONNEGATIVE}\fi}

\def\drawdotedge#1#2{\zzcnA=0\zzdmA=0pt\zzdmB=#1
\zzcheckposdimen\zzdmB{}{DRAWDOTEDGE}\zzcheckbool{#2}{SECOND}{DRAWDOTEDGE}
\zzdrawedge{\zzcnG=\zzcnC\divide\zzcnG by \zzcnE\relax
\ifnum\zzcnG<1\relax\zzcnG=1\fi\zzcnE=\zzcnC\divide\zzcnE by \zzcnG\relax
\ifnum#2=0\relax\advance\zzcnG by -1\fi}
{\kern-1.39pt\raise-.76pt\hbox{.}}}

\def\drawsolidedge{\zzcnA=1\zzdmA=0pt\zzdmB=0pt
\zzdrawedge{\zzcnG=0\zzcnD=\zzcnC}
{\line(\xslope,\yslope){\zzcnD}}}

\def\zzdrawedge#1#2{\zzcheckedge{DRAW}\relax
\ifnum\zzcnA=1\relax\zzcheckslope\xslope\yslope 6{SOLID OR DASHED EDGE}\fi
\zzcnA=\xstart\zzcnB=\ystart\zzcnD=\zzdmA\zzcnE=\zzdmB\relax
\ifnum\xslope=0\relax\zzcnC=\yend\advance\zzcnC by -\zzcnB\zzcnF=\yslope
\else\zzcnC=\xend\advance\zzcnC by -\zzcnA\zzcnF=\xslope
\zzdistance\xslope\yslope\relax
\ifnum\xslope<0\relax\global\zzglobalcnA=-\zzglobalcnA\fi
\multiply\zzcnD by 100\divide\zzcnD by \zzglobalcnA\multiply\zzcnD by \xslope
\multiply\zzcnE by 100\divide\zzcnE by \zzglobalcnA\multiply\zzcnE by \xslope
\fi
\ifnum\zzcnF<0\relax\zzcnC=-\zzcnC\fi
\ifnum\zzcnC>0\relax #1\relax
\ifnum\zzcnF<0\relax\zzcnE=-\zzcnE\fi\zzcnF=\zzcnE\relax
\ifnum\xslope=0\relax\zzcnE=0
\else\multiply\zzcnF by \yslope\divide\zzcnF by \xslope\fi
\zzmakepicture{\loop\put(\zzcnA,\zzcnB){#2}
\ifnum\zzcnG>0\relax\advance\zzcnG by -1
\advance\zzcnA by \zzcnE\advance\zzcnB by \zzcnF\repeat
\zzrecordwidth\xstart\xstart\zzrecordwidth\xend\xend
\zztotheight=\ystart\zztotdepth=\ystart\zzrecordheight\yend\yend}\fi}

%

\def\drawedgehead#1#2#3{\zzcheckbool{#2}{SECOND}{DRAWEDGEHEAD}
\zzcheckbool{#3}{THIRD}{DRAWEDGEHEAD}\zzcnB=#3
\relax\ifnum#2=1\relax\zzcnA=#1\relax
\zzdrawedgeheada\xstart\ystart\xend\yend\xslope\yslope
\else\zzcnA=100\advance\zzcnA by -#1\relax
\zzdrawedgeheada\xend\yend\xstart\ystart{-\xslope}{-\yslope}\fi}

%

\def\zzcheckbool#1#2#3{
\ifnum#1<0\errmessage{#2 PARAMETER OF #3 MUST BE 1 OR 0}\fi
\ifnum#1>1\errmessage{#2 PARAMETER OF #3 MUST BE 1 OR 0}\fi}

\def\zzdrawedgeheada#1#2#3#4#5#6{\zzcheckedge{DRAW ARROWHEAD FOR}
\zzcheckslope{#5}{#6}4{ARROWHEAD}
\zzdmA=#3\advance\zzdmA by -#1
\divide\zzdmA by 10\multiply\zzdmA by \zzcnA\divide\zzdmA by 10
\zzdmB=#4\advance\zzdmB by -#2
\divide\zzdmB by 10\multiply\zzdmB by \zzcnA\divide\zzdmB by 10
\relax\ifnum\zzcnB=1\relax
\zzdistance{#5}{#6}\zzdmC=\edgeheaddisp
\multiply\zzdmC by 100\divide\zzdmC by \zzglobalcnA\zzdmD=\zzdmC
\multiply\zzdmC by #5\multiply\zzdmD by #6
\advance\zzdmA by \zzdmC\advance\zzdmB by \zzdmD\fi
\advance\zzdmA by #1\zzcnA=\zzdmA\advance\zzdmB by #2\zzcnB=\zzdmB
\zzmakepicture{\put(\zzcnA,\zzcnB){\vector(#5,#6){0}}
\zzrecordwidth\zzdmA\zzdmA\zztotheight=\zzdmB\zztotdepth=\zzdmB}}

%
%

\def\zzcheckslope#1#2#3#4{\relax
\ifnum#1>#3\zzcheckslopea{#1}{#2}{#4}\fi
\ifnum#1<-#3\zzcheckslopea{#1}{#2}{#4}\fi
\ifnum#2>#3\zzcheckslopea{#1}{#2}{#4}\fi
\ifnum#2<-#3\zzcheckslopea{#1}{#2}{#4}\fi}

\def\zzcheckslopea#1#2#3{\errmessage{\the#1,\the#2 IS ILLEGAL SLOPE FOR #3}}

%
%
%
%
%
%
%

\def\abutleft#1:#2#3{\zzabut{#1}{#2}{#3}{-\yslope}{\zzslidehoriz}{1}}
\def\abutright#1:#2#3{\zzabut{#1}{#2}{#3}{\yslope}{\zzslidehoriz}{1}}
\def\abutbelow#1:#2#3{\zzabut{#1}{#2}{#3}{\xslope}{\zzslidevert}{1}}
\def\abutabove#1:#2#3{\zzabut{#1}{#2}{#3}{-\xslope}{\zzslidevert}{1}}

\def\abutleftd#1#2#3{\zzabut{#1}{#2}{#3}{-\yslope}{\zzslidehoriz}{0}}
\def\abutrightd#1#2#3{\zzabut{#1}{#2}{#3}{\yslope}{\zzslidehoriz}{0}}
\def\abutbelowd#1#2#3{\zzabut{#1}{#2}{#3}{\xslope}{\zzslidevert}{0}}
\def\abutaboved#1#2#3{\zzabut{#1}{#2}{#3}{-\xslope}{\zzslidevert}{0}}

\def\zzabut#1#2#3#4#5#6{\zzcheckedge{ABUT TO}
\zzsetupbox{#2}{#3}\zzcnA=\xslope\zzcnB=\yslope
\relax\ifnum#4<0\relax\zzcnA=-\zzcnA\zzcnB=-\zzcnB\fi
\def\zzprocpoly{\zzclosestpoly}\def\zzprocrorect{\zzprocrorecta}
\zzglobalshadow
\advance\zzdmC by -\zzglobalxcenter\advance\zzdmD by -\zzglobalycenter
\relax\ifnum#6=1\relax\zzmultdiagramunit\zzdmA{#1}\else\zzdmA=#1\fi
\zzdmB=\zzdmA#5\relax\zzissue}

\def\zzslidehoriz{\relax\ifnum\yslope=0\errmessage
{ABUTLEFT OR ABUTRIGHT ATTEMPTED FOR HORIZONTAL EDGE}\fi
\advance\zzdmA by \zzdmD\advance\zzdmA by -\ystart
\multiply\zzdmA by \xslope\divide\zzdmA by \yslope
\advance\zzdmA by \xstart\advance\zzdmA by -\zzdmC}

\def\zzslidevert{\relax\ifnum\xslope=0\errmessage
{ABUTBELOW OR ABUTABOVE ATTEMPTED FOR VERTICAL EDGE}\fi
\advance\zzdmB by \zzdmC\advance\zzdmB by -\xstart
\multiply\zzdmB by \yslope\divide\zzdmB by \xslope
\advance\zzdmB by \ystart\advance\zzdmB by -\zzdmD}

%
%
%
%
%
%
%

\def\zzclosestpoly#1#2#3{\zzdmC=#1\zzdmD=#2\zzcnC=0\zzclosestpolya #3\end}

\def\zzclosestpolya#1{\def\zztesta{#1}\def\zztestb{\end}
\ifx\zztesta\zztestb\let\zznext=\zzclosestpolyb
\else\let\zznext=\zzclosestpolyc\fi\zznext {#1}}

\def\zzclosestpolyb#1{}

\def\zzclosestpolyc#1#2#3{\zzcnD=\zzcnB\multiply\zzcnD by #1\relax
\zzcnE=\zzcnA\multiply\zzcnE by #2\relax\advance\zzcnD by -\zzcnE\relax
\ifnum\zzcnD>0\relax
\ifnum\zzcnC=1\let\zznext=\zzclosestpolyd
\else\zzcnC=0\zzcastpolyd{#1}{#2}{#3}\let\zznext=\zzclosestpolya\fi
\else\zzcnC=1\zzcastpolyd{#1}{#2}{#3}\let\zznext=\zzclosestpolya\fi
\zznext}

\def\zzclosestpolyd#1\end{}

%
%

\def\setcircle#1#2#3{\dcircle=#1\xcircle=#2\ycircle=#3\zziscircle=1}

%

\def\shiftcircle#1#2{\zzcheckcircle{SHIFT}
\advance\xcircle by #1\advance\ycircle by #2}

\def\zzcheckcircle#1{\relax\ifnum\zziscircle=0\errmessage
{ATTEMPT TO #1 NONEXISTENT CIRCLE}\fi}

%

\def\drawcircle#1#2#3#4{\zzcheckcircle{DRAW}\zzdmA=\dcircle\divide\zzdmA by 2
\zzmakepicture{\zzcnA=\dcircle\zzcnB=\xcircle\zzcnC=\ycircle
\zztotheight=\ycircle\zztotdepth=\ycircle
\zzrecordwidth\xcircle\xcircle\relax
\zzdrawcirclea{#1}{tr}{\zzdmA}{\zzdmA}\zzdrawcirclea{#2}{br}{\zzdmA}{-\zzdmA}
\zzdrawcirclea{#3}{bl}{-\zzdmA}{-\zzdmA}
\zzdrawcirclea{#4}{tl}{-\zzdmA}{\zzdmA}}}

\def\zzdrawcirclea#1#2#3#4{\zzcheckbool{#1}{}{DRAWCIRCLE}\ifnum#1=1\relax
\put(\zzcnB,\zzcnC){\oval(\zzcnA,\zzcnA)[#2]}
\zzdmB=\xcircle\advance\zzdmB by #3\zzrecordwidth\zzdmB\zzdmB
\zzdmB=\ycircle\advance\zzdmB by #4\zzrecordheight\zzdmB\zzdmB\fi}

%

\def\drawcirclehead#1#2#3{\zzcheckcircle{DRAW ARROWHEAD FOR}
\zzreduceterms{#1}{#2}{0,0 ARE ILLEGAL PARAMETERS FOR DRAWCIRCLEHEAD}
\zzdistance{\zzcnC}{\zzcnD}\zzcheckbool{#3}{THIRD}{DRAWCIRCLEHEAD}
\ifnum#3=1\relax\zzcnA=\zzcnD\zzcnB=-\zzcnC\else\zzcnA=-\zzcnD\zzcnB=\zzcnC\fi
\zzdmA=\dcircle\multiply\zzdmA by 50\divide\zzdmA by \zzglobalcnA
\zzdmB=\circleheaddisp\multiply\zzdmB by 100\divide\zzdmB by \zzglobalcnA
\zzdmE=\zzdmA\multiply\zzdmE by \zzcnC\zzdmC=\xcircle\advance\zzdmC by \zzdmE
\zzdmE=\zzdmB\multiply\zzdmE by \zzcnA\advance\zzdmC by \zzdmE
\zzdmE=\zzdmA\multiply\zzdmE by \zzcnD\zzdmD=\ycircle\advance\zzdmD by \zzdmE
\zzdmE=\zzdmB\multiply\zzdmE by \zzcnB\advance\zzdmD by \zzdmE
\zzcnC=\zzdmC\zzcnD=\zzdmD\zzcheckslope\zzcnA\zzcnB4{ARROWHEAD}
\zzmakepicture{\put(\zzcnC,\zzcnD){\vector(\zzcnA,\zzcnB){0}}
\zzrecordwidth\zzdmC\zzdmC\zztotheight=\zzdmD\zztotdepth=\zzdmD}}

%
%

\def\abutcircleleft#1#2#3{\zzabutcircle{#1}{#2}{#3}{}
\zzslidehoriz{\relax\ifdim\zzdmA>\zzdmH\relax\zzdmH=\zzdmA\fi}}

\def\abutcircleright#1#2#3{\zzabutcircle{#1}{#2}{#3}{\zzrotate\zzrotate}
\zzslidehoriz{\relax\ifdim\zzdmA<\zzdmH\relax\zzdmH=\zzdmA\fi}}

\def\abutcirclebelow#1#2#3{\zzabutcircle{#1}{#2}{#3}{\zzrotate}
\zzslidevert{\relax\ifdim\zzdmB>\zzdmI\relax\zzdmI=\zzdmB\fi}}

\def\abutcircleabove#1#2#3{\zzabutcircle
{#1}{#2}{#3}{\zzrotate\zzrotate\zzrotate}
\zzslidevert{\relax\ifdim\zzdmB<\zzdmI\relax\zzdmI=\zzdmB\fi}}

\def\zzabutcircle#1#2#3#4#5#6{\zzcheckcircle{ABUT TO}
\zzsetupbox{#2}{#3}\def\zzprocpoly{\zzclosestpoly}
\def\zzprocrorect{\zzprocrorecta}
\zzdmF=\dcircle\divide\zzdmF by 2
\zzdmG=\dcircle\multiply\zzdmG by 100\divide\zzdmG by 283
\xstart=-\zzdmF\ystart=0pt\xslope=0\yslope=-1
\zzabutcirclea{#1}{#4}{#5}\zzdmH=\zzdmA\zzdmI=\zzdmB
\xstart=-\zzdmG\ystart=\zzdmG\xslope=-1\yslope=-1
\zzabutcirclea{#1}{#4}{#5}#6\relax
\xstart=-\zzdmG\ystart=-\zzdmG\xslope=1\yslope=-1
\zzabutcirclea{#1}{#4}{#5}#6\relax
\zzdmA=\zzdmH\advance\zzdmA by \xcircle
\zzdmB=\zzdmI\advance\zzdmB by \ycircle
\zzissue}

\def\zzabutcirclea#1#2#3{#2\relax
\zzcnA=\xslope\zzcnB=\yslope
\zzglobalshadow
\advance\zzdmC by -\zzglobalxcenter\advance\zzdmD by -\zzglobalycenter
\zzdmA=#1\zzdmB=\zzdmA #3\relax}

\def\zzrotate{\zzdmE=\xstart\xstart=-\ystart\ystart=\zzdmE
\zzcnC=\xslope\xslope=-\yslope\yslope=\zzcnC}

%

%
\def\ctvertexstyle{\displaystyle}
\def\ctabutstyle{\textstyle}
\def\ctvertexborderlr{3pt}
\def\ctvertexbordertb{4pt}
\def\ctloopdiameter{20pt}
\def\ctabutcircledisp{5pt}
\def\ctabutborderlr{2pt}
\def\ctabutbordertb{2pt}
\def\ctabutborderinset{3pt}
\def\ctabutborderinsetdouble{6pt}%
\def\ctdoubleedgedisp{2pt}

%
\newdimen\zzdmX\newdimen\zzdmY

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%

\def\ctdiagram#1{\diagram{\ctsolid\cthead\ctoutermid #1}}

%
%
%
%
%
%

\def\ctvg#1,#2:#3#4{\vertex #1,#2:{\ctvertexstyle #3}{#4\relax
\border\ctvertexborderlr\ctvertexbordertb\rect}}

\def\ctv#1,#2:#3{\ctvg #1,#2:{#3}{}}

%
%

\def\ctgl#1{\leftghost{\ctvertexstyle #1}}

\def\ctgr#1{\rightghost{\ctvertexstyle #1}}

%
%
%

\def\ctlptl#1{\zzctlp{\lexpr\texpr}{{0pt}\circleheaddisp}{1011}{101}
{\abutcircleleft\ctabutcircledisp}{#1}}

\def\ctlptlcc#1{\zzctlp{\lexpr\texpr}{{-\circleheaddisp}{0pt}}{1011}{0{-1}0}
{\abutcircleleft\ctabutcircledisp}{#1}}

\def\ctlptr#1{\zzctlp{\rexpr\texpr}{\circleheaddisp{0pt}}{1101}{0{-1}1}
{\abutcircleright\ctabutcircledisp}{#1}}

\def\ctlptrcc#1{\zzctlp{\rexpr\texpr}{{0pt}\circleheaddisp}{1101}{{-1}00}
{\abutcircleright\ctabutcircledisp}{#1}}

\def\ctlpbr#1{\zzctlp{\rexpr\bexpr}{{0pt}{-\circleheaddisp}}{1110}{{-1}01}
{\abutcircleright{-\ctabutcircledisp}}{#1}}

\def\ctlpbrcc#1{\zzctlp{\rexpr\bexpr}{\circleheaddisp{0pt}}{1110}{010}
{\abutcircleright{-\ctabutcircledisp}}{#1}}

\def\ctlpbl#1{\zzctlp{\lexpr\bexpr}{{-\circleheaddisp}{0pt}}{0111}{011}
{\abutcircleleft{-\ctabutcircledisp}}{#1}}

\def\ctlpblcc#1{\zzctlp{\lexpr\bexpr}{{0pt}{-\circleheaddisp}}{0111}{100}
{\abutcircleleft{-\ctabutcircledisp}}{#1}}

\def\zzctlp#1#2#3#4#5#6{\border\ctvertexborderlr\ctvertexbordertb
\setcircle\ctloopdiameter #1
\border{-\ctvertexborderlr}{-\ctvertexbordertb}
\shiftcircle #2\drawcircle #3\drawcirclehead #4
#5{\ctabutstyle #6}\zzctabutprog}

\def\zzctabutprog{\border\ctabutborderlr\ctabutbordertb
\borderto{\ctabutborderinsetdouble}{\ctabutborderinsetdouble}
\octagon\ctabutborderinset}

%
%

\def\cten#1:{\setedge#1:\shadeedge\zzctdrawedge\zzctdrawhead1}

%
%

\def\ctet#1:#2{\setedge#1:\zzctxmean\zzcte\abutaboved{#2}\zzctxmeanadj}

\def\cteb#1:#2{\setedge#1:\zzctxmean\zzcte\abutbelowd{#2}\zzctxmeanadj}

\def\ctel#1:#2{\setedge#1:\zzctymean\zzcte\abutleftd{#2}\zzctymeanadj}

\def\cter#1:#2{\setedge#1:\zzctymean\zzcte\abutrightd{#2}\zzctymeanadj}

\def\zzctxmean{\zzdmX=\xstart\advance\zzdmX by \xend\divide\zzdmX by 2}

\def\zzctymean{\zzdmX=\ystart\advance\zzdmX by \yend\divide\zzdmX by 2}

\def\zzcte#1#2#3{\shadeedge #3\zzctdrawedge\zzctdrawhead1
#1\zzdmX{\ctabutstyle #2}\zzctabutprog}

%
%

\def\ctetg#1;#2:#3{\setedge#1:\zzmultdiagramunit\zzdmX{#2}\zzcte
\abutaboved{#3}\relax}

\def\ctebg#1;#2:#3{\setedge#1:\zzmultdiagramunit\zzdmX{#2}\zzcte
\abutbelowd{#3}\relax}

\def\ctelg#1;#2:#3{\setedge#1:\zzmultdiagramunit\zzdmX{#2}\zzcte
\abutleftd{#3}\relax}

\def\cterg#1;#2:#3{\setedge#1:\zzmultdiagramunit\zzdmX{#2}\zzcte
\abutrightd{#3}\relax}

%
%
%

\def\ctetb#1:#2#3#4#5{\zzcheckbool{#2}{FIFTH}{CTETB}
\zzcheckbool{#3}{SIXTH}{CTETB}
\setedge#1:\zzctxmean\zzctee\xslope\abutaboved\abutbelowd
{#2}{#3}{#4}{#5}\zzctxmeanadj}

\def\ctelr#1:#2#3#4#5{\zzcheckbool{#2}{FIFTH}{CTELR}
\zzcheckbool{#3}{SIXTH}{CTELR}
\setedge#1:\zzctymean\zzctee\yslope\abutleftd\abutrightd
{#2}{#3}{#4}{#5}\zzctymeanadj}

\def\ctetbg#1;#2,#3:#4#5#6#7{\zzcheckbool{#4}{SEVENTH}{CTETBG}
\zzcheckbool{#5}{EIGHTH}{CTETBG}\setedge#1:\zzmultdiagramunit\zzdmX{#2}
\zzctee\xslope
\abutaboved{\zzmultdiagramunit\zzdmX{#3}\abutbelowd}{#4}{#5}{#6}{#7}\relax}

\def\ctelrg#1;#2,#3:#4#5#6#7{\zzcheckbool{#4}{SEVENTH}{CTELRG}
\zzcheckbool{#5}{EIGHTH}{CTELRG}\setedge#1:\zzmultdiagramunit\zzdmX{#2}
\zzctee\yslope
\abutleftd{\zzmultdiagramunit\zzdmX{#3}\abutrightd}{#4}{#5}{#6}{#7}\relax}

\def\zzctee#1#2#3#4#5#6#7#8{
\ifnum#1>0\relax\zzdmY=\ctdoubleedgedisp\else\zzdmY=-\ctdoubleedgedisp\fi
\shiftedge\zzdmY\shadeedge #8\zzctdrawedge\zzctdrawhead{#4}
#2\zzdmX{\ctabutstyle #6}\zzctabutprog
\multiply\zzdmY by -2\relax
\shiftedge\zzdmY\shadeedge #8\zzctdrawedge\zzctdrawhead{#5}
#3\zzdmX{\ctabutstyle #7}\zzctabutprog}

%
%
%
%

\def\ctinnermid{\def\zzctxmeanadj{\zzctxmean}\def\zzctymeanadj{\zzctymean}}

\def\ctoutermid{\def\zzctxmeanadj{\relax}\def\zzctymeanadj{\relax}}

%

\def\zzctdrawdashedge{\relax
\ifnum\xslope=0\relax\drawdashedge{7pt}{7pt}11
\else\ifnum\yslope=0\relax\drawdashedge{7pt}{7pt}11
\else\drawdashedge{15pt}{7pt}01\fi\fi}

%

\def\zzctdrawdotedge{\drawdotedge{8pt}1}

%
%
%

\def\ctsolid{\def\zzctdrawedge{\drawsolidedge}}

\def\ctdash{\def\zzctdrawedge{\zzctdrawdashedge}}

\def\ctdot{\def\zzctdrawedge{\zzctdrawdotedge}}

%
%
%

\def\zzctdrawedgehead#1{\relax\ifnum#1=1\relax
\drawedgehead{100}10\else\drawedgehead{0}00\fi}

\def\zzctnodrawedgehead#1{}

%
%

\def\cthead{\def\zzctdrawhead{\zzctdrawedgehead}}

\def\ctnohead{\def\zzctdrawhead{\zzctnodrawedgehead}}


==> parameters-acm.tex <==
\def\OPTIONArxiv{0}
\def\OPTIONAppendix{0}

